Successor Heads: Recurring, Interpretable Attention Heads In The Wild

In this work we present successor heads: attention heads that increment tokens with a natural ordering, such as numbers, months, and days. For example, successor heads increment 'Monday' into 'Tuesday'. We explain the successor head behavior with an approach rooted in mechanistic interpretability, the field that aims to explain how models complete tasks in human-understandable terms. Existing research in this area has found interpretable language model components in small toy models. However, results in toy models have not yet led to insights that explain the internals of frontier models and little is currently understood about the internal operations of large language models. In this paper, we analyze the behavior of successor heads in large language models (LLMs) and find that they implement abstract representations that are common to different architectures. They form in LLMs with as few as 31 million parameters, and at least as many as 12 billion parameters, such as GPT-2, Pythia, and Llama-2. We find a set of 'mod-10 features' that underlie how successor heads increment in LLMs across different architectures and sizes. We perform vector arithmetic with these features to edit head behavior and provide insights into numeric representations within LLMs. Additionally, we study the behavior of successor heads on natural language data, identifying interpretable polysemanticity in a Pythia successor head.

==> sections/1_introduction.tex <==
% \section{Introduction}
% \label{sec:intro}

% Mechanistic interpretability \citep{AnthropicMechanisticEssay} involves reverse-engineering the algorithms that trained neural networks have learnt.
% A lot of recent attention has been paid to interpreting transformer-based large language models (LLMs), as while these models have impressive capabilities \citep{gpt4}, there is little understanding into how these models produce their outputs.
% Existing interpretability research includes comprehensive reverse-engineering efforts into toy models \citep{nanda2023progress} and small language models \citep{olsson2022context,wang2023interpretability}, though few conclusions have been made about how frontier LLMs function.
% In this work, we find an interpretable set of attention heads we call \vocab{Successor Heads} in models of many different scales and architectures.
% We find Successor Heads in the smallest and largest Pythia language models \citep{biderman2023pythia}, that have between 30 million and 12 billion parameters.
% We can understand the role of Successor Heads through concise paths in models (\Cref{fig:successor_head_main_fig}) and we identify transferrable features that these attention heads use across different tasks (\Cref{sec:interp_successor}).

% % Can we put the residual stream arrows in this diagram? %
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/intro/main_succ.pdf} % use https://latex2image.joeraut.com/ and https://lucid.app/lucidchart/404e1ac0-e94c-4093-8a4d-1ce51bb7aad7/edit?viewport_loc=495%2C-265%2C1314%2C618%2C0_0&invitationId=inv_53eac781-2669-4cbd-b296-dcd62ed93aa6
%     \caption{Successor Heads lie on a length 3 path through models. This consists of three linear transformations in \textbf{\textcolor{brown}{beige}} and one non-linearity in \textbf{\textcolor{gray}{gray}}. We show evidence that residual connections are not important in \Cref{app:residual}}
%     \label{fig:successor_head_main_fig}
% \end{figure}

% In mechanistic interpretability, universality \citep{olah2020zoom, li2016convergent} is a hypothesis that there are \textit{common representations} in neural networks. 
% The universality hypothesis firstly asserts that neural networks with different architectures and \textit{scales} form common representations. 
% It also asserts that different downstream \textit{tasks} use common representations. 
% Importantly, strong evidence for or against the universality hypothesis could significantly affect research priorities in interpretability.
% If common representations form across different language models, then research on small or toy language models \citep{elhage2022toy, elhage2021mathematical}, as well as research on narrow natural language tasks \citep{wang2023interpretability, docstring, greaterthan} may be the best way to gain insights into LLM capabilities.
% Conversely, if the representations used by language models do not generalize to different models scales and/or tasks, then developing methods that can be applied to larger language models (e.g \citet{geiger_alignment}, \citet{bills2023language}, \citet{conmy2023automated}) may be the most important direction for interpretability.
% In this work, we find evidence for a weak form of universality (\citet{bilal}) in language models, as
% \begin{compactenum}
%     \item Successor Heads use a \textit{common representation}, such as a `mod 10' direction in activation space.
%     \item Successor Heads form across language models from the \textit{scale} of 31 million parameters and to at least as many as 12 billion parameters.
%     \item Successor Heads perform incrementation across several different \textit{tasks}.
% \end{compactenum}

% Successor Heads are attention heads that perform incrementation in language models.
% The input to a successor head is the representation of a token with a numeric meaning, such as `Monday', `first', `January' or `one'.
% The output of a successor head is the increased likelihood of the incremented token, such as `Tuesday', `second, `February' or `two'.
% We operationalize Successor Heads formally in \Cref{sec:successor_heads}.
% Surprisingly, we find that across many language models of different architectures and sizes, successor heads perform incrementation across several numeric tasks, suggesting that language models can use common abstractions for different tasks, which we mechanistically explain in \Cref{sec:interp_successor}.
% Additionally, Successor Heads are important for incrementation on natural language training data, though they also perform other tasks, some of which are interpretable (\Cref{sec:in_the_wild}).
% Altogether, main contributions of our work are:
% \begin{compactenum}
%     \item Defining and surveying Successor Heads in many autoregressive language models (\Cref{sec:successor_heads}).
%     \item Finding abstract cross-task representations of numbers that are linearly represented in model activations (\Cref{sec:interp_successor}). 
%     \item Showing that Successor Heads are important for incrementation token completions in natural language training datasets (\Cref{sec:in_the_wild}).
% \end{compactenum}
